One-shot Learning for Temporal Knowledge Graphs

Most real-world knowledge graphs are characterized by a long-tail relation frequency distribution where a significant fraction of relations occurs only a handful of times. This observation has given rise to recent interest in low-shot learning methods that are able to generalize from only a few examples. The existing approaches, however, are tailored to static knowledge graphs and not easily generalized to temporal settings, where data scarcity poses even bigger problems, e.g., due to occurrence of new, previously unseen relations. We address this shortcoming by proposing a one-shot learning framework for link prediction in temporal knowledge graphs. Our proposed method employs a self-attention mechanism to effectively encode temporal interactions between entities, and a network to compute a similarity score between a given query and a (one-shot) example. Our experiments show that the proposed algorithm outperforms the state of the art baselines for two well-studied benchmarks while achieving significantly better performance for sparse relations.

==> sections/archive.tex <==
\section{Important Issues}
\textcolor{red}{The main issue with the rare geopolitical event forecasting is not the model, but the lacking of a good ground truth. As we have seen in our experiments, ICEWS dataset is not a good representative of the real world events. The real world rare events might not be rare in ICEWS, like Kim Jong-Un meeting Trump that was recorded as many events in the dataset during the course of two month. Also the rare relations in ICEWS might be just noise. For example when looking at low-level CAMEO code for an IFP related to nuclear war, we observed a couple of nuclear ICEWS events during the past 6 month!
Therefor, training and evaluating the model on ICEWS dataset reduces the few-shot forecasting problem to a rare link prediction task on ICEWS dataset and even a perfect model with $100\%$ performance is predicting ICEWS events.
Besides, a simple linear tensor forecasting model has already shown promising results. The meta learning model suggested above might be too complicated and over-parameterized for this task.}
Given the above issues, I can think of following options: 
\begin{enumerate}
\item We don't limit our application to only ICEWS dataset and geopolitcal event forecasting. Instead, we define the problem as rare link prediction on dynamic knowledge graphs. There are other dynamic knowledge graphs, that could be used for experiments, such as YAGO, FREEBASE and WIKIDATA.  
\item We can do aggregation on top of ICEWS events, to get more realistic events. For example instead of many events related to Kim Jong-Un meeting during two month, we aggregate them into one event. The question is, how are we going to evaluate our aggregation approach. 

\item Add other geopolitical and social media datasets. 

\end{enumerate}

\section{Potential Future Research}
\begin{enumerate}
    \item \textbf{Change The Baseline Model.} There exists a lot of distance learning and similarity based meta learning models that can be replaced with ``Matching Networks'' used in the baseline model, for example: \cite{snell2017prototypical}, that could improve the performance in rare link prediction on knowledge graphs.
    
    \item \textbf{Speed up Graph Embedding Methods with Meta Learning.} The idea behind optimization based meta learning approaches is to learn a model that could generalize across tasks. So let say we are given a set of tasks $\mathcal{T} = \{T_1, \dots, T_k \}$. Instead of optimizing for each task and learning parameters $\{\theta_1 \dots \theta_k\}$, we learn a generalized parameter $\theta$ that could work across all the tasks. Now let say each task $T_i$ is to learn an embedding on a random sub-graph of a graph $G$. Can we use meta learning to learn optimal model parameters for a general graph embedding on $G$ with less training steps? A similar idea is recently proposed in \cite{ostapuk2019activelink}. 
    
    % \item \textbf{Considering Node Hierarchies In ICEWS Dataset} Our models for embedding ICEWS dataset only considers countries. Other papers in the literature that studied link prediction on ICEWS dataset, consider actor names. Would a hierarchical embedding help to improve the performance? \textcolor{red}{This is very incremental}
    
\end{enumerate}{}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{l || c c c c | c c c c}
        \toprule
        & \multicolumn{4}{c|}{GDELT} & \multicolumn{4}{c}{ICEWS} \\
        \cline{2-9}
        Model & H@1 & H@5 & H@10 & MRR & H@1 & H@5 & H@10 & MRR\\
        \midrule
        TTransE  &.011/.011 &.034/.064 &.046/.117 &.033/.047&.011/.000 & .066/.047 & .110/.091 & .050/.035\\
        TATransE &.000/.000 &.172/.255 &.241/.372 &.081/.119 & .000/.000 & .253/.178 &.406/ .363 & .122/098\\
        ReNet & .092/.064 & .149/.191&.207/.319 & .136/.146 & .197/.126 & .549/.289 & .637/.407 & .369/.209\\
        \midrule
        GMatching &.037/.007 &.067/.037 & .085/.067&.055/.028 & .100/.062 & .298/.156 & .360/.233 & .193/.113\\
        FSRL &.110/.080 &.149/.158 &.168/.210 & .144/.127 & .204/.120 & .356/.253 & .430/.345 &.280/.192\\
        MetaR & .000/.003& .197/.235 & .243/.293& .091/.115 & .116/.044 &.374/.172 &.477/.244 & .240/.112\\
        \midrule
        % TempFewShot + mean & & & & & 0.058 & 0.151 & 0.290 & 0.142 \\
        TempFewShot &.071/.058 &\textbf{.180}/.148 &\textbf{.417}/\textbf{.352} & \textbf{.166}/\textbf{.147} & .149/\textbf{.138} & .433/\textbf{.405} & .607/\textbf{.654} & .273/\textbf{.269} \\
        
        \bottomrule
    \end{tabular}
    }
\caption{Hit@k results for one-shot learning ($k=1$) on (i) one month of GDELT (Jan 2018) and (ii) two years of ICEWS (Jan 2017 - Jan 2019) for VAL/Test meta relations.}
\label{tab:icews_results}
\end{table*}

 \begin{table}[h!]
     \centering
     \begin{tabular}{c|c c }
        \toprule
            \backslashbox{Model}{Metric} & MRR & H@10  \\
        \midrule
            M1&.168/220&.356/.518\\
            M2 &.269/.245&.593/.616\\
        \midrule
          Full Model&.273/.269&.607/.654\\
        \bottomrule
     \end{tabular}
     \caption{Ablation study results}
     \label{tab:ablation}
 \end{table}
 
 
 \begin{table*}[t]
\centering

    \begin{tabular}{l c || c c c c | c c c c}
        \toprule
        & & \multicolumn{4}{c|}{GDELT} & \multicolumn{4}{c}{ICEWS} \\
        \cline{3-10}
        Model& Suppot& H@1 & H@5 & H@10 & MRR & H@1 & H@5 & H@10 & MRR\\
        \midrule
        TTransE  & train &0.011 &0.064 &0.117 &0.047&0.000 & 0.047 & 0.091 & 0.035\\
        TATransE & train & 0.000 &0.192 &0.329 &0.101 & 0.000 & 0.178 & 0.363 & 0.098\\
        ReNet & train & 0.064 & 0.191&0.319 & 0.146 & 0.126 & 0.289 & 0.407 & 0.209\\
        \midrule
        GMatching & test &0.007 &0.037 & 0.067& 0.028 & 0.062 & 0.156 & 0.233 & 0.113\\
        FSRL & test & 0.080 & 0.158 & 0.210 & 0.127 & 0.120 & 0.253 & 0.345 & 0.192\\
        MetaR & test & .0.003& 0.235 & 0.293& 0.115 & 0.044 & 0.172 & 0.244 & 0.112\\
        \midrule
        % TempFewShot + mean & & & & & 0.058 & 0.151 & 0.290 & 0.142 \\
        TempFewShot & test & 0.058 &0.148 &0.352 & 0.147 & \textbf{0.138} & \textbf{0.405} & \textbf{0.654} & \textbf{0.269} \\
        TempFewShot & train & 0.060 &0.155 &\textbf{0.365} & 0.146 & 0.132 & 0.394 & 0.639 & 0.264 \\
        \bottomrule
    \end{tabular}
    
\caption{Hit@k results for one-shot learning ($k=1$) on (i) one month of GDELT (Jan 2018) and (ii) two years of ICEWS (Jan 2017 - Jan 2019) for Test meta relations.}
\label{tab:icews_results}
\end{table*}

% @inproceedings{nickel2016holographic,
%   title={Holographic embeddings of knowledge graphs},
%   author={Nickel, Maximilian and Rosasco, Lorenzo and Poggio, Tomaso},
%   booktitle={Thirtieth Aaai conference on artificial intelligence},
%   year={2016}
% }


% @inproceedings{nickel2011three,
%   title={A three-way model for collective learning on multi-relational data.},
%   author={Nickel, Maximilian and Tresp, Volker and Kriegel, Hans-Peter},
%   booktitle={ICML},
%   volume={11},
%   pages={809--816},
%   year={2011}
% }
% @inproceedings{socher2013reasoning,
%   title={Reasoning with neural tensor networks for knowledge base completion},
%   author={Socher, Richard and Chen, Danqi and Manning, Christopher D and Ng, Andrew},
%   booktitle={Advances in neural information processing systems},
%   pages={926--934},
%   year={2013}
% }
% @inproceedings{dettmers2018convolutional,
%   title={Convolutional 2d knowledge graph embeddings},
%   author={Dettmers, Tim and Minervini, Pasquale and Stenetorp, Pontus and Riedel, Sebastian},
%   booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
%   year={2018}
% }

% @inproceedings{trouillon2016complex,
%   title={Complex embeddings for simple link prediction},
%   author={Trouillon, Th{\'e}o and Welbl, Johannes and Riedel, Sebastian and Gaussier, {\'E}ric and Bouchard, Guillaume},
%   year={2016},
%   booktitle={International Conference on Machine Learning (ICML)}
% }

% @inproceedings{yang2014embedding,
%   title={Embedding entities and relations for learning and inference in knowledge bases},
%   author={Yang, Bishan and Yih, Wen-tau and He, Xiaodong and Gao, Jianfeng and Deng, Li},
%   booktitle={ICLR},
%   year={2014}
% }

% @inproceedings{bordes2013translating,
%   title={Translating embeddings for modeling multi-relational data},
%   author={Bordes, Antoine and Usunier, Nicolas and Garcia-Duran, Alberto and Weston, Jason and Yakhnenko, Oksana},
%   booktitle={Advances in neural information processing systems},
%   pages={2787--2795},
%   year={2013}
% }


 
% @inproceedings{schlichtkrull2018modeling,
%   title={Modeling relational data with graph convolutional networks},
%   author={Schlichtkrull, Michael and Kipf, Thomas N and Bloem, Peter and Van Den Berg, Rianne and Titov, Ivan and Welling, Max},
%   booktitle={European Semantic Web Conference},
%   pages={593--607},
%   year={2018},
%   organization={Springer}
% }
 






==> sections/background.tex <==
\section{Problem Formulation}

We present the formal definition of a TKG and explore few-shot learning tasks for temporal link prediction. 

\subsection{Temporal Knowledge Graph Completion}
A TKG can be represented as a set of quadruples $G = \{(s, r, o, t) | s, o \in \mathcal{E}, r \in \mathcal{R} \}$, where $\mathcal{E}$ is the set of entities, $\mathcal{R}$ is the set of relations and $t$ is the timestamp. Graph completion for a static KG involves predicting new facts by either predicting an unseen object entity for a given subject and relation $(s, r, ?)$ or predicting an unseen link between the subject and object entity $(s, ? , o)$. In this work, we are interested in the former case, but at a particular timestamp $t$. More formally, we want to predict new events $(s, r, ?, t)$ at time $t$ by ranking the true object entities higher than others by a scoring function $\mathcal{P}$, parameterized by a neural network and its value indicating the event likelihood. %The likelihood of an event is conditioned on the 
The key idea in  modeling the temporal events is that an event likelihood depends on the events in the previous $l$ timesteps $\{t-l, \dots, t-2, t-1\}$. In Section~\ref{sec:model_encoder} we explain in detail that how temporal information is encoded in our model. 

\subsection{Few-shot Learning and Episodic Training}
Few-shot Learning (FSL) focuses on building and training a model with only a few labeled instances for each class. Meta-learning is a framework to address FSL where we incorporate a large set of tasks, each task mimicking an \textit{N-way K-shot} classification scenario, and leverage the shared information across the tasks to compensate for the scarcity of information about each task resulting from having few labeled data points. %FSL should also rapidly generalize to new classes using a few labeled samples. 

The idea of episodic training for meta-learning is to match the training procedure with the inference at test time~\cite{vinyals2016matching}. More specifically, consider that we have a large set of tasks $\mathcal{T}$. Each episode consists of a subset of tasks $L$, sampled from $\mathcal{T}$, a support set $S$, and a batch $B$ both sampled from $L$. Note that both $S$ and $B$ are labeled examples, labels coming from $L$. The goal is to train a model that maps the few examples in the support set into a classifier. The probabilistic optimization objective for this problem can be formulated as:

\small
\begin{equation}
\theta = \underset{\theta}{\argmax} E_{L \sim \mathcal{T}} \Bigg[ E_{S\sim L, B \sim L}\Bigg[ \underset{(x, y) \in B}{\sum} \log P_{\theta}(y | x, S) \Bigg]\Bigg].
\label{temp}
\end{equation}
 \normalsize
 
We adopt the standard episodic training framework in Eq.~\eqref{temp} for the purpose of TKG completion.

\subsection{Few-shot TKG Setup}
\label{sec:fewshot-setup}
As mentioned earlier, data scarcity is even a bigger problem in relational learning with TKGs. Few-shot episodic training has been proven to be effective to tackle this problem for static KGs~\cite{xiong2018one}. We further extend the framework proposed by Xiong et al.~\citeyear{xiong2018one} for TKG completion. 

Given a TKG, $G = \{(s, r, o, t) | s, o \in \mathcal{E}, r \in \mathcal{R} \}$, the relations of $\mathcal{R}$ are divided into two groups based on their frequency: frequent relations $\mathcal{F}$ and sparse relations $\mathcal{T}$. The sparse relations are used to build the task set needed by the model for the episodic training. Each task is a defined as a sparse relation $r \in \mathcal{T}$ and has its own training and test set, denoted and support and query set and defined as follows:
\begin{equation}
\begin{split}
&S_r^t = \{(s_i, r, o_i, t_i) | s_i, o_i\in\mathcal{E}\}_{i=1}^{k}\\
&Q_r^t = \{(s_q, r, o_q, t_q) | s_q, o_q\in\mathcal{E}, t_q \in [t, t + w]\},
\end{split}
\end{equation}

where $t = \max\{t_i\}_{i=1}^k$. Note that unlike static graphs, where each relation was considered as a task and the choice of support and query set was random, here the timestamps of the quadruples selected for the query set are restricted by their distance from the support timestamp. 
%selecting the query set and the support set is restricted by timestamp. 
Figure~\ref{fig:query} illustrates  the time constraint used for selecting the query examples. More details on sampling procedure for the support and query set are provided in Section~\ref{sec:training}. The parameter $w$ is called the \textit{episode length}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/query.png}
%     \caption{The support set includes a set of consecutive events, assuming that $t_i$ is the timestamp of the last quadruple in the support set, the query examples are selected from $[t_i, t_i + w]$   }
%     \label{fig:query}
% \end{figure}{}


The loss function $l_{\theta}$ at each episode optimizes a score function $\mathcal{P_{\theta}}$ such that for a given test query in $Q_r^t$, the true object entities are ranked higher than the others. The score function is a metric space learnt during the training, and the score represents the  similarity between a test query and the support set representation. The  final optimization loss   is:
\begin{equation}
\mathcal{L} = E_{r \sim \mathcal{T} } \bigg[ E_{Q_r^t \sim G, S_r^t \sim G} \bigg[ l_{\theta}(Q_r^t | S_r^t)\bigg] \bigg] 
\end{equation}

 The relations in $\mathcal{T}$ are divided into train, validation and test relations, called $\mathcal{T}_{meta-train}, \mathcal{T}_{meta-test}, \mathcal{T}_{meta-val}$ respectively. Note that any pair of these sets are mutually exclusive. To make the temporal setup more representative of the real world, we do not assume any time overlap between the quadruples in the \textit{meta-train}, \textit{meta-val} and \textit{meta-test}. Figure \ref{fig:split} depicts the time split for meta-train, meta-validation and meta-test. To have the episodes in the training match with the inference,  the split window for validation and test is equal to $w$.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/split.png}
%     \caption{Meta-train, Meta-validation and Meta-test split across time}
%     \label{fig:split}
% \end{figure}

\begin{figure}
    \centering
    
    \begin{subfigure}[t]{0.5\textwidth}
        \begin{tikzpicture}[scale=1, transform shape]
    % draw horizontal line   
    \draw[ultra thick, ->] (0,0) -- (\textwidth,0);
    
    % draw vertical lines
    \foreach \x in {0.5,1.5,2.5,3.5,4.5,5.5,6.5,7.5}
    \draw (\x cm,3pt) -- (\x cm,-3pt);
    
    
    \draw[thick, -latex] (7.5, 0) -- (7.5, 0.7)node[xshift=0.25cm, above,thick] {\shortstack{Event: \\$(s, r, o, t)$} };
    \draw[thick, -latex] (1.5, 0) -- (1.5, 0.7);
    \draw[thick, -latex] (4.5, 0) -- (4.5, 0.7);
    \draw[thick, -latex] (6.5, 0) -- (6.5, 0.7);
    
    % draw node
    \draw[ultra thick] (7.5,0) node[below=3pt,thick] {$t$ } node[above=3pt] {};
    \draw[ultra thick] (6.5,0) node[below=3pt,thick] {$t-1$} node[above=3pt] {};
    \draw[ultra thick] (4.5,0) node[below=3pt,thick] {$t-3$} node[above=3pt] {};
    \draw[ultra thick] (2.5,0) node[below=5pt,thick] {$\dots\dots$} node[above=3pt] {};
    \draw[ultra thick] (0.5,0) node[below=3pt,thick] {$t-l$} node[above=3pt] {};
    


    \draw [ black, ultra thick,decorate,decoration={brace,mirror, amplitude=5pt},
           yshift=-5pt] (0.5,-0.5) -- (6.6,-0.5)
           node [black,midway,below=4pt] {History};
           
    
    \end{tikzpicture}
    \caption{Event history}
    \label{fig:history}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.5\textwidth}
        \begin{tikzpicture}[scale=1, transform shape]
    % draw horizontal line   
    \draw[ultra thick, ->] (0,0) -- (\textwidth,0);
    
    % draw vertical lines
    \foreach \x in {0.5,1.5,2.5,3.5,4.5,5.5,6.5,7.5}
    \draw (\x cm,3pt) -- (\x cm,-3pt);
    
    \draw[thick, -latex] (1.5, 0) -- (1.5, 0.7);
    \draw[thick, -latex] (2.5, 0) -- (2.5, 0.7)node[xshift=0.25cm, above,thick] {$(s_i, r, o_i, t_i)$ };
    \draw[thick, -latex] (4.5, 0) -- (4.5, 0.7);
    \draw[thick, -latex] (6.5, 0) -- (6.5, 0.7);
    
    % draw node
    \draw[ultra thick] (7.5,0) node[below=3pt,thick] {$t_i + w$ } node[above=3pt] {};
    \draw[ultra thick] (2.5,0) node[below=3pt,thick] {$t_i$} node[above=3pt] {};
    


    \draw [ black, ultra thick,decorate,decoration={brace,mirror, amplitude=5pt},
           yshift=-5pt] (2.8,-0.5) -- (7.6,-0.5)
           node [black,midway,below=4pt] {\footnotesize  $Q_r^{t_i}$};
           
    \draw [ black, ultra thick,decorate,decoration={brace,mirror, amplitude=5pt},
           yshift=-5pt] (0.3,-0.5) -- (2.7,-0.5)
           node [black,midway,below=4pt] {\footnotesize $S_r^{t_i}$};
    
    \end{tikzpicture}
    \caption{Query and support set construction}
    \label{fig:query}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.5\textwidth}
        \begin{tikzpicture}[scale=1, transform shape]
    % draw horizontal line   
    \draw[ultra thick, ->] (0,0) -- (\textwidth,0);
    
    % draw vertical lines
    \foreach \x in {0.5,4.5,6,7.5}
    \draw (\x cm,3pt) -- (\x cm,-3pt);
    
    % draw node
    \draw[ultra thick] (0.5,0) node[above=3pt,thick] {Start} node[above=3pt] {};
    \draw[ultra thick] (7.5,0) node[above=3pt,thick] {End} node[above=3pt] {};

    
    \draw [ black, ultra thick,decorate,decoration={brace,mirror, amplitude=8pt},
           yshift=-2pt] (0.4,-0.5) -- (4.5,-0.5)
           node [black,midway,below=4pt] {\footnotesize  $Meta_{train}$};
           
    \draw [ black, ultra thick,decorate,decoration={brace,mirror, amplitude=8pt},
          yshift=-2pt] (4.5,-0.5) -- (6,-0.5)
          node [black,midway,below=4pt] {\footnotesize $Meta_{val}$};
    
    \draw [ black, ultra thick,decorate,decoration={brace,mirror, amplitude=8pt},
           yshift=-2pt] (6,-0.5) -- (7.6,-0.5)
           node [black,midway,below=4pt] {\footnotesize $Meta_{test}$};
    \end{tikzpicture}
    \caption{Train, validation and test split across time}
    \label{fig:split}
    \end{subfigure}
    \caption{(a) Neighborhood encoder extracts the information from $l$ previous timestamps $[t-l, t-1]$ (b) The query set is selected from $[t_i, t_i + w]$, with $t_i$ being the last quads timestamp in the support (c) There is no time overlap between quadruples in validation and test.}
    \label{fig:my_label}
    \vspace{-1em}
\end{figure}

Finally, we assume that the model has access to a background knowledge graph defined as $G' = \{(s, r, o, t) | s, o\in\mathcal{E}, r \in \mathcal{F}\}$, and the entity set $\mathcal{E}$ is a closed set, i.e., there are no unseen entities during the inference time. 



==> sections/table_country.tex <==
\begin{table*}[t]
\centering
\caption{Hit@k results for one-shot ($k=1$) model with matching network for  $l = 10$ and $w = 120$ days on \textcolor{red}{XXX} of GDELT dataset from \textcolor{red}{XXX}  to \textcolor{red}{XXX} }
\vspace{0.3 cm}
\centering
    \begin{tabular}{l || c c c c | c c c c}
        \toprule
         & \multicolumn{4}{c|}{GDELT-COUNTRY} & \multicolumn{4}{c}{GDELT-ACTOR} \\
        \cline{2-9}
        Model & H@1 & H@5 & H@10 & MRR & H@1 & H@5 & H@10 & MRR\\
        \midrule
        \midrule
        TTransE & & & & &.011/.011 &.034/.064 &.046/.117 &.033/.047\\
        TATransE  & & & & &.000/.000 &.172/.255 &.241/.372 &.081/.119\\
        ReNet & & & & &.092/.064 & .149/.191&.207/.319 & .136/.146\\
        \midrule
        GMatching & & & & &.037/.007 &.067/.037 & .085/.067&.055/.028 \\
        FSRL & & & & &.110/.080 &.149/.158 &.168/.210 & .144/.127\\
        MetaR & & & & & .000/.003& .197/.235 & .243/.293& .091/.115\\
        \midrule
        TempFewShot & & & & &.071/.058 &\textbf{.180}/.148 &\textbf{.417}/\textbf{.352} & \textbf{.166}/\textbf{.147}\\
        
        \bottomrule
    \end{tabular}
    
\label{tab:gdelt_results}
\end{table*}

% 
% 
